Accelerated Wirtinger Flow for Multiplexed Fourier Ptychographic Microscopy

Fourier ptychographic microscopy enables gigapixel-scale imaging, with both large field-of-view and high resolution. Using a set of low-resolution images that are recorded under varying illumination angles, the goal is to computationally reconstruct high-resolution phase and amplitude images. To increase temporal resolution, one may use multiplexed measurements where the sample is illuminated simultaneously from a subset of the angles. In this paper, we develop an algorithm for Fourier ptychographic microscopy with such multiplexed illumination. Specifically, we consider gradient descent type updates and propose an analytical step size that ensures the convergence of the iterates to a stationary point. Furthermore, we propose an accelerated version of our algorithm (with the same step size) which significantly improves the convergence speed. We demonstrate that the practical performance of our algorithm is identical to the case where the step size is manually tuned. Finally, we apply our parameter-free approach to real data and validate its applicability.

==> backup/Section2_mahdi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proposed Model
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Forward Model} \label{Sec:Method}
We start with the mathematical description of the measurement formation process
in FPM with multiplexed coded illumination. We consider the setup in
Figure~\ref{fig:Setup} where an array of light-emitting diodes (LEDs) is used
as the illumination source of a standard microscope. The coordinate vector is
given by $(\rbf,z)$ where $\rbf = (r_1,r_2) \in \R^2$ denotes the spatial
location on a transverse plane perpendicular to the optical axis $z$. A
\textit{thin} sample (that is the 2D object to be imaged) is located at
$z=0$, which is the rear focal plane of the objective. 

The sample is characterized by a complex-valued \textit{transmission function} 
\begin{align}
  s(\rbf) \coloneqq \sqrt{I(\rbf)} \exp\left(
  \cj \phi(\rbf) \right)\hspace{-.23em}\text{,} 
  \label{eq:objectField}
\end{align}
where the continuous mappings $I:\Omega\rightarrow \R$ and
$\phi:\Omega\rightarrow \R$ represent the spatial \textit{intensity} and
\textit{phase} maps (of the sample), respectively. Here, the domain $\Omega$ is
assumed to be a compact subset of $\R^2$.

Placing the LED array sufficiently far away,  each LED
illumination is modeled by a monochromatic plane wave at the sample plane
$z=0$. When the $i$th LED is switched on, the field
exiting the sample (and entering the microscope objective) is given by
$
s_{i} (\rbf) = s(\rbf) \exp \left( 2 \pi \cj \langle \xibf_{i}, \rbf
\rangle \right),
$ 
where $\xibf_{i}$ is the spatial frequency vector of the corresponding angle of
illumination\footnote{$\xibf_{i} \coloneqq (1/\lambda)( \cos(\alpha_{i}),
\cos(\beta_{i}))$ where $\lambda$ is the wavelength; $\alpha_{i}$ and
$\beta_{i}$ are the angles of incidence on the axes $r_1$ and $r_2$,
respectively.}. In effect, each $s_i$ is uniquely described by shifting the
Fourier transform\footnote{The Fourier transform $\hat{f}$ of a function $f$ is
defined by 
\begin{align*}
  \widehat{f}(\xibf) = \mathcal{F} \lbr f \rbr (\xibf) &\coloneqq \iint
  f(\rbf) \exp\left( -\cj 2 \pi \langle \xibf,\rbf \rangle \right)
  \dint\rbf\text{.}
\end{align*}
} of the transmission function $\widehat{s}$ since it holds that
$ 
  \widehat{s_{i}} (\cdot) = \widehat{s} (\cdot - \xibf_{i})\text{.} 
$

Due to the finite-aperture objective lens, the exit field is low-pass filtered
as it goes though the microscope. The process is specified by the
\textit{pupil} function $\widehat{p}$, that is the Fourier transform of the
coherent point spread function, and suppresses special frequencies beyond the
diffraction limit. Consequently, the camera captures the intensity of the
lower-resolution field and the measurement is expressed by
\begin{equation}
  I_{i}(\rbf) = \Bigl \lvert \Fo^{-1} \lbr \left(\widehat{p}(\cdot) \,
  \widehat{s}(\cdot - \xibf_{i}) \right) \rbr \Bigr\lvert^2(\rbf) \text{.} 
  \label{eq:measuredImage}
\end{equation}
We see in~\eqref{eq:measuredImage} that FPM can sample spatial frequency
bands---up to the phase information that is lost during the
acquisition---beyond the diffraction limit via angle-varying illumination.
Rather than turning on LEDs on one at a time, \textit{multiplexed} measurements
are used to speed up the data acquisition. In this case, a subset of LEDs are
simultaneously lit. Since LEDs are mutually incoherent with each other, the
total intensity of the multiplexed measurement is expressed as the sum of the
intensity if each LED was switched on individually:
\begin{equation}
  I_{\mathcal{M}}(\rbf) =  \sum_{i \in \mathcal{M}} I_i (\rbf)\text{,} 
  \label{eq:multiplexedImage}
\end{equation}
where $\mathcal{M}$ denotes the index set of the selected LEDs.

%\begin{align*}
%  \widehat{p} (\xibf) \coloneqq \left\{
%    \begin{array}{ll}
%      1 \quad \text{if} \quad  \abs{\xibf} \leq \lambda/{\rm NA}_{\rm obj}
%      \text{;}\\ 
%      0 \quad \text{otherwise,}\\ 
%    \end{array}
%  \right.
%  \label{eq:pupilFunction}
%\end{align*}
%where ${\rm NA_{obj}}$ is the numerical aperture (NA) of the objective lens.

%However, since the phase information is lost during the acquisition, the
%sampled frequency bands significantly overlap to facilitate a stable recovery.
%This redundancy  

\begin{figure}[t]
  \centering
  \includegraphics[width=0.485\textwidth]{figs/scheme_setup.pdf}
  \caption{Representation of the optical setup and the corresponding problem
  geometry. Multiple LEDs  simultaneously illuminate the sample that is located
  at the input plane of a microscope objective. Sample's image is generated at
  the camera plane where intensity-only measurements are recorded.}
  \label{fig:Setup}
\end{figure}

Finally, we discretize~\eqref{eq:multiplexedImage} by considering its
\textit{amplitude-based} counterpart as such formulations are more robust to
both noise and model mismatch~\cite{Yeh.etal2015}. To that end, let $\sbf
\in\C^{n}$ be a discretization of the Fourier transform of the transmission
function and $\ybf_{\mathcal{M}} \in \R^{m}_{\geq 0}$ the discrete samples of
$\sqrt{I_{\mathcal{M}}}$ at pixel locations. We  note that  $m < n$ since the
reconstructed transmission function has a higher space-bandwidth product than
the measured image.  For each multiplexed measurement, the discretized forward
model is hence given by
\begin{equation}
  \ybf_{\mathcal{M}} = \sqrt{\sum_{i \in \mathcal{M}} \,\abs{ \Fbf\cT \Pbf
  \Cibf \sbf }^2} \text{.} 
  \label{eq:discreteForwardModel}
\end{equation}
where $\Cibf \in \C^{m \times n}$ is the matrix representation of the $m$-pixel
cropping centered at $\xibf_{i}$, $\Pbf \in \C^{m \times m}$ is a diagonal
matrix generated from the discretized pupil function, and $\Fbf\cT \in \C^{m
\times m}$ represents the discrete inverse Fourier transform. We also note that
$\abs{\cdot}^2$ and $\sqrt{\cdot}$ are entry-wise operations.

%Finally, we consider a discretized forward model that is the
%\textit{amplitude-based} counterpart of~\eqref{eq:multiplexedImage}. To this
%aim let $\mtx{s}\in\C^{N_1\times N_2}$ be an $N_1\times N_2$ discretization of
%the Fourier transform of the object. Then the discretized measurements are
%given by 
%\begin{equation}
%%\lvert \Fbf  \cT \Pbf \Slbf \sbf 
%  \ybf_{\mathcal{L}} = \sqrt{\sum_{\ell \in \mathcal{L}} \,\abs{\Fo_{n_1\times
%  n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2} \text{.} 
%  \label{eq:discreteForwardModel}%
%\end{equation}
%Here, $\mtx{p}\in\C^{n_1\times n_2}$ is an $n_1\times n_2$ discretization of
%the Fourier transform of the pupil function, $\mathcal{S}_\ell:\C^{N_1\times
%N_2}\rightarrow \C^{n_1\times n_2}$ is a mapping that when applied to
%$\mtx{s}\in\C^{N_1\times N_2}$ crops an $n_1\times n_2$ window with center
%located at position $\xibf_{\ell}$, $\Fo_{n_1\times n_2}^{-1}:\C^{n_1\times
%n_2}\rightarrow \C^{n_1\times n_2}$ represents the $n_1\times n_2$ discrete
%inverse Fourier transform, and $\odot$ represents entry-wise or Hadamard
%product between the two matrices. Also, for a matrix $\mtx{M}\in\C^{n_1\times
%n_2}$, $\abs{\mtx{M}}^2$ denotes a matrix of size $n_1\times n_2$ whose
%$ij$-th entry is given by $\abs{\mtx{M}_{ij}}^2$, i.e.~ $\abs{\cdot}^2$ should
%be interpreted as being applied entry by entry. Finally, $\ybf_{\mathcal{L}}
%\in \R^{n_1\times n_2}$ denotes the discretized samples of
%$\sqrt{I_{\mathcal{L}}}$.
%
%In~\eqref{eq:discreteForwardModel}, $\ybf_{\mathcal{L}} \in \R^N$ ($N$ denotes
%the number of pixels) is the vectorized representation of the samples of
%$\sqrt{I_{\mathcal{L}}}$ at pixel locations. $\Fbf \in \C^{N
%\times N}$ is the discrete Fourier transform (DFT) matrix, $\Pbf \in \R^{N
%\times N}$ is a binary diagonal matrix that representing the response of the
%microscope, $\Slbf \in \R^{N \times N}$ is a shift matrix specified by
%$\xibf_{\ell}$, and $\widehat{\sbf} \in \C^N$ is the vectorized discrete
%Fourier transform of the transmission function. 

\section{Reconstruction Algorithm: Accelerated Wirtinger Flow}
In this section we propose a reconstruction algorithm for recovering the
sample's amplitude and phase maps from a set of multiplexed measurements. To
this aim, we solve the following optimization problem:
\begin{align}
\label{opt}
&\underset{\mbf{s}\in\C^{n}}{\text{minimize}}\quad \mathcal{J}(\mbf{s})\quad\text{with}\nonumber\\
&\quad\quad\mathcal{J}(\mbf{s}) \coloneqq \sum_{k=1}^K \twonorm{\ybf_{\mathcal{M}_k} - \sqrt{\sum_{i \in \mathcal{M}} \,\abs{ \Fbf\cT \Pbf
  \Cibf \sbf }^2} }^2
%\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\ell\left(\sqrt{\mtx{I}^{(k)}_{i,j}},\abs{[\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)]_{ij}}\right).%\mathcal{R}(\vct{z})\le \mathcal{R}(\vct{x}).
\end{align}
Here, $K$ represents the total number of captured multiplexed images. We note that the above cost measures the discrepancy between the measurements and the output of the model given by \eqref{eq:discreteForwardModel}. A natural approach to solve this problem is via gradient descent type updates of the form
%\begin{align*}
%\mathcal{K}=\{\vct{w}\in\R^n:\mathcal{R}(\vct{w})\le \mathcal{R}(\vct{x})\}.
%\end{align*}
\begin{align}
\label{iters}
\vct{s}_{\tau+1}=\vct{s}_\tau-\mu_\tau\nabla \mathcal{C}(\vct{s}_\tau),
\end{align}
with $\mu_\tau$ the learning rate. We note that since $\mathcal{C}(\vct{s})$ is a mapping from $\mathbb{C}^{n_1\times n_2}$ to $\R$, it is not holomorphic and hence not complex-differentiable. However, it is still possible to define a gradient based on the notion of Wirtinger derivatives.  Following \cite{WF} we shall refer to the iterates \eqref{iters} as Wirtinger Flow. The loss function in \eqref{opt} is not differentiable and a-priori it may not be clear how to run Wirtinger Flow in this case. However, this does not pose a fundamental challenge as the loss function is differentiable except for isolated points and we can use the notion of generalized gradients to define the gradient at a non-differentiable point as one of the limits points of the gradient in a local neighborhood of the non-differentiable point. For the loss in \eqref{opt} the generalized gradient takes the form
\begin{align}
\label{gengrad}
&\nabla \mathcal{L}(\vct{s}):=\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\widetilde{\mathcal{S}}_{\ell}\left(\bar{\vct{p}}\odot \Fo_{n_1\times n_2}\left(\vct{e}\right)\right)\quad\text{where}\nonumber\\
&\vct{e}=\left(\sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2}-\ybf_{\mathcal{L}_k} \right)\odot\nonumber\\
&\quad\quad\left(\frac{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}{\sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2}}\right).
%&\sum_{k=1}^K \bar{\vct{p}}_k\odot\mathcal{F}^*\left(\left(\sqrt{\mtx{I}^{(k)}}-\abs{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}\right)\odot\frac{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}{\abs{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}}\right).
\end{align}
%%\begin{algorithm}[t]
%%    \caption{Accelerated Wirtinger Flow (AWF)}
%%    \label{AWF}
%%    \begin{algorithmic}
%%    \STATE{\bfseries Input:} Measurements $\ybf_{\mathcal{L}}$, Fourier transform of the probe $\vct{p}$ and center shifts $\xibf_\ell$ for different displacements of the probe. 
%%    \STATE {\bfseries Parameters:} $T$ iterations ($\tau$)
%%   \STATE {\bfseries Initialize:}  $\vct{s}_1=\vct{1}_{N_1\times N_2}$ or a random matrix
%%   \FOR{$\tau=1$ \textbf{to} $T$}
%%   \STATE 
%%   \vspace{-0.5cm}
%%   \begin{align*}
%%   \vct{s}_{\tau+1}\leftarrow&\vct{s}_\tau+\beta_\tau\left(\vct{s}_\tau-\vct{s}_{\tau-1}\right)\\
%%   &\quad\quad\quad-\mu_\tau\nabla \mathcal{C}\left(\vct{s}_\tau+\beta_\tau\left(\vct{s}_\tau-\vct{s}_{\tau-1}\right)\right)
%%   \end{align*}
%%   \STATE with 
%%   \vspace{-0.5cm}
%%\begin{align*}
%%&\nabla \mathcal{L}(\vct{s}):=\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\widetilde{\mathcal{S}}_{\ell}\left(\bar{\vct{p}}\odot \Fo_{n_1\times n_2}\left(\vct{e}\right)\right)\quad\text{where}\nonumber\\
%%&\vct{e}=\left(\sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2}-\ybf_{\mathcal{L}_k} \right)\odot\nonumber\\
%%&\quad\quad\left(\frac{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}{\sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2}}\right),
%%%&\sum_{k=1}^K \bar{\vct{p}}_k\odot\mathcal{F}^*\left(\left(\sqrt{\mtx{I}^{(k)}}-\abs{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}\right)\odot\frac{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}{\abs{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}}\right).
%%\end{align*}
%%   \STATE 
%%   $\beta_\tau=\frac{\tau+1}{\tau+3},$ and
%%   $\mu_\tau = \frac{1}{ \infnorm{\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}\odot \abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}}}$.
%%   \ENDFOR 
%%    \STATE{\bfseries Output:} $\vct{s}_T$
%%    \end{algorithmic}
%%  \end{algorithm}
Here, $\bar{\mtx{p}}\in\C^{n_1\times n_2}$ is a matrix whose entries are the conjugate of the entries of $\mtx{p}$ and $\Fo_{n_1\times n_2}:\C^{n_1\times n_2}\rightarrow \C^{n_1\times n_2}$ represents the $n_1\times n_2$ two dimensional discrete Fourier transform. Also, $\widetilde{\mathcal{S}}_\ell:\C^{n_1\times n_2}\rightarrow \C^{N_1\times N_2}$ is a mapping that when applied to $\mtx{x}\in\C^{n_1\times n_2}$ creates an all zero matrix of size $N_1\times N_2$ except for a submatrix of size $n_1\times n_2$ with center located at position $\xibf_{\ell}$ which is set to $\vct{x}$. Furthermore, for two matrices $\mtx{A}$ and $\mtx{B}$ of the same size $\frac{\mtx{A}}{\mtx{B}}$ is used to denote element-wise division. In particular, $\frac{\mtx{A}}{\abs{\mtx{A}}}$ is a matrix whose entries contain the phase of the entries of the matrix $\mtx{A}$. We propose the following step size for the Wirtinger Flow iterates
\begin{align}
\label{step1}
\mu_\tau =\mu:=\frac{1}{ \infnorm{\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}\odot \abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}}}.
\end{align}
Here, for a matrix $\mtx{A}$, $\infnorm{\mtx{A}}$ denotes the maximum absolute value of the entries of $\mtx{A}$ i.e.~$\infnorm{\mtx{A}}:=\max_{ij}\abs{\mtx{A}_{ij}}$. We shall demonstrate in Section \ref{Sec:NumericalResults} that the Wirtinger Flow iterates \eqref{iters} using the generalized gradient in \eqref{gengrad} enjoys faster convergence when compared with many classical phase retrieval schemes. This result holds with the step size \eqref{step1}. However, the convergence rate is still rather slow. To overcome this challenge, inspired by \cite{} we apply the accelarted iterations
\begin{align}
\label{AWF}
\vct{s}_{\tau+1}=\vct{s}_\tau+\beta_\tau\left(\vct{s}_\tau-\vct{s}_{\tau-1}\right)-\mu_\tau\nabla \mathcal{C}\left(\vct{s}_\tau+\beta_\tau\left(\vct{s}_\tau-\vct{s}_{\tau-1}\right)\right).
\end{align}
Following \cite{} we shall refer to these iterations as Accelarated Wirtinger Flow (AWF). We also propose the following values for the parameters $\beta_\tau$ and $\mu_\tau$ so that our approach requires no tuning parameters
\begin{align}
\label{params}
\beta_\tau=&\frac{\tau+1}{\tau+3}\quad\text{and}\quad\nonumber\\
\mu_\tau =&\mu:=\frac{1}{ \infnorm{\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}\odot \abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}}}.
\end{align}
%We summarize this approach in Algorithm \ref{AWF}.

We note that Nesterov's accelerated scheme applies to convex and smooth functions. However, the loss function in \eqref{opt} is neither convex nor differentiable. Therefore, a-priori it is not clear why such an accelerated scheme is useful. Perhaps unexpectedly, we shall demonstrate in Section \ref{Sec:NumericalResults} that these accelerated iterates not only enjoy much faster convergence but also reach better optima!

\section{Theory for convergence to stationary points}
\label{sectheory}
In this section we wish to provide some theoretical justification for our choice of the learning rates \eqref{step1} and \eqref{params} for Wirtinger Flow and Accelerated Wirtinger Flow.
\begin{theorem}\label{mainthm} For $k=1,2,\ldots,K$, let $\ybf_{\mathcal{L}_k}\in\mathbb{R}^{n_1\times n_2}$ denote arbitrary measurements. Also let $\vct{p}\in\mathbb{C}^{n_1\times n_2}$ denote the discretized Fourier transform of the probe. We run the Wirtinger Flow updates
\begin{align*}
\vct{s}_{\tau+1}=\vct{s}_\tau-\mu_\tau\nabla\mathcal{C}(\vct{s}_\tau),
\end{align*}
with $\nabla \mathcal{C}(\vct{s})$ as defined in \eqref{gengrad} and learning rate $\mu_\tau$  obeying
\begin{align}
\label{stepthm}
\mu_\tau =\mu:=\frac{1}{ \infnorm{\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}\odot \abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}}}.
\end{align}
Also let $\vct{s}_{*}\in\underset{\vct{s}\in\C^{N_1\times N_2}}{\arg\min} \mathcal{C}(\vct{s})$ be a global optima. Then, the following identities hold
\begin{align*}
\underset{\tau\rightarrow\infty}{\lim} \fronorm{\nabla \mathcal{C}(\vct{s}_\tau)}\rightarrow 0,
\end{align*}
and
\begin{align*}
\min_{\tau\in\{1,2,\ldots,T\}} \fronorm{\nabla \mathcal{C}(\vct{s}_\tau)}^2\le \frac{\left(\mathcal{C}(\vct{s}_1)-\mathcal{C}(\vct{s}_{*})\right)}{\mu T}.
\end{align*}
\end{theorem}
This theorem demonstrates that with our chosen step size the Wirtinger Flow iterates converge to a point where the generalized gradient is zero. This is a non-trivial statement as the loss function is none smooth and there are many stationary points where the generalized gradient does not vanish. The main use of this theorem in this paper is that it allows us to select the learning rate properly. We would like to note that this theorem does not show convergence to a local optimum. Furthermore, this theorem does not provide convergence guarantees for Accelerated Wirtinger Flow. We hope to address such questions in our future work. 


==> expand_ <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proposed Model
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section{Forward Model} \label{Sec:Method}
We start with an overview of the mathematical description of the measurement
formation process in FPM. In doing so, we consider the setup depicted in
Figure~\ref{fig:Setup} where an array of light-emitting diodes (LEDs) is used
to obtain coded multiplexed illumination. The coordinate vector is given by
$(\rbf,z)$ where $\rbf = (r_1,r_2) \in \R^2$ denotes the spatial location on a
transverse plane perpendicular to the optical axis $z$. A \textit{thin} sample
(that is the 2D object to be imaged) is located at $z=0$, which is the rear
focal plane of the microscope objective. 

The sample is characterized by a complex-valued \textit{transmission function} 
\begin{align}
  s(\rbf) \coloneqq \sqrt{I(\rbf)} \exp\left(
  \cj \phi(\rbf) \right)\hspace{-.23em}\text{,} 
  \label{eq:objectField}
\end{align}
where the continuous mappings $I:\Omega\rightarrow \R$ and
$\phi:\Omega\rightarrow \R$ represent the spatial \textit{intensity} and
\textit{phase} maps of the sample, respectively. Here, the domain $\Omega$ is
assumed to be compact subset of $\R^2$.


Placing the LED array sufficiently far away from the sample,  each LED
illumination is modeled by a monochromatic plane wave at the sample plane
$z=0$. We note that when the $i$th LED is switched on, the electric field
exiting the sample is given by
$
s_{i} (\rbf) = s(\rbf) \exp \left( 2 \pi \cj \langle \xibf_{i}, \rbf
\rangle \right),
$ 
where $\xibf_{i}$ is the spatial frequency vector specified by the
corresponding angle of illumination~\footnote{$\xibf_{i} \coloneqq (1/\lambda)(
\cos(\alpha_{i}), \cos(\beta_{i}))$ where $\lambda$ is the wavelength;
$\alpha_{i}$ and $\beta_{i}$ are the angles of incidence on the axes $r_1$ and
$r_2$, respectively.}. This implies that each exit field is described by
shifting the Fourier transform~\footnote{The Fourier transform $\hat{f}$ of a
function $f$ is defined by 
\begin{align*}
  \widehat{f}(\xibf) = \mathcal{F} \lbr f \rbr (\xibf) &\coloneqq \iint
  f(\rbf) \exp\left( -\cj 2 \pi \langle \xibf,\rbf \rangle \right)
  \dint\rbf\text{.}
\end{align*}
} of the tranmission function $\widehat{s}$ since
\begin{align} 
  \widehat{s_{i}} (\cdot) = \widehat{s} (\cdot - \xibf_{i})\text{.} 
  \label{eq:shiftInFourier}
\end{align}
Since the sample is at the input plane of the microscope,  each exit field $s_{\ell}$ then passes through the microscope, where it is
low-pass filtered (due to diffraction) by the pupil function 
\begin{align*}
  \widehat{p} (\xibf) \coloneqq \left\{
    \begin{array}{ll}
      1 \quad \text{if} \quad  \abs{\xibf} \leq \lambda/{\rm NA}_{\rm obj}
      \text{;}\\ 
      0 \quad \text{otherwise,}\\ 
    \end{array}
  \right.
  \label{eq:pupilFunction}
\end{align*}
where ${\rm NA_{obj}}$ is the numerical aperture (NA) of the objective lens.
The camera captures only the intensity of this low-resolution object so that
the measured image is specified by
\begin{equation}
  I_{\ell}(\rbf) = \Bigl \lvert \Fo^{-1} \lbr \left(\widehat{p}(\cdot) \,
  \widehat{s}(\cdot - \xibf_{\ell}) \right) \rbr \Bigr\lvert^2(\rbf) \text{.} 
  \label{eq:measuredImage}
\end{equation}

As for the multiplexed coded illumination case, a chosen subset of LEDs are
simultaneously lit instead of turning them on one at a time. Since LEDs on the
array are mutually incoherent with each other, the total intensity is simply
the sum of the intensity if each LED was switched on individually. In this
case, the measured image becomes 
\begin{equation}
  I_{\mathcal{L}}(\rbf) =  \sum_{\ell \in \mathcal{L}} \, \Bigl \lvert \Fo^{-1}
  \lbr \left(\widehat{p}(\cdot) \, \widehat{s}(\cdot - \xibf_{\ell}) \right)
  \rbr \Bigr\lvert^2(\rbf) \text{,} 
  \label{eq:multiplexedImage}
\end{equation}
where $\mathcal{L}$ denotes the index set of the selected LEDs.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.485\textwidth]{figs/scheme_setup.pdf}
  \caption{Representation of the optical setup and the corresponding problem
  geometry. Multiple LEDs  simultaneously illuminate the sample from
  different angles. The sample is located at the input plane of a microscope
  objective and its magnified image is generated at the camera plane. Note
  that the camera captures intensity-only measurements, necessitating phase
  retrieval.}
  \label{fig:Setup}
\end{figure}

Finally, we consider a discretized forward model that is the
\textit{amplitude-based} counterpart of~\eqref{eq:multiplexedImage}. To this aim let $\mtx{s}\in\C^{N_1\times N_2}$ be an $N_1\times N_2$ discretization of the Fourier transform of the object. Then the discretized measurements are given by 
\begin{equation}
%\lvert \Fbf  \cT \Pbf \Slbf \sbf 
  \ybf_{\mathcal{L}} = \sqrt{\sum_{\ell \in \mathcal{L}} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2} \text{.} 
  \label{eq:discreteForwardModel}%
\end{equation}
Here, $\mtx{p}\in\C^{n_1\times n_2}$ is an $n_1\times n_2$ discretization of the Fourier transform of the pupil function, $\mathcal{S}_\ell:\C^{N_1\times N_2}\rightarrow \C^{n_1\times n_2}$ is a mapping that when applied to $\mtx{s}\in\C^{N_1\times N_2}$ crops an $n_1\times n_2$ window with center located at position $\xibf_{\ell}$, $\Fo_{n_1\times n_2}^{-1}:\C^{n_1\times n_2}\rightarrow \C^{n_1\times n_2}$ represents the $n_1\times n_2$ discrete inverse Fourier transform, and $\odot$ represents entry-wise or Hadamard product between the two matrices. Also, for a matrix $\mtx{M}\in\C^{n_1\times n_2}$, $\abs{\mtx{M}}^2$ denotes a matrix of size $n_1\times n_2$ whose $ij$-th entry is given by $\abs{\mtx{M}_{ij}}^2$, i.e.~ $\abs{\cdot}^2$ should be interpreted as being applied entry by entry. Finally, $\ybf_{\mathcal{L}} \in \R^{n_1\times n_2}$ denotes the discretized samples of $\sqrt{I_{\mathcal{L}}}$.

%In~\eqref{eq:discreteForwardModel}, $\ybf_{\mathcal{L}} \in \R^N$ ($N$ denotes
%the number of pixels) is the vectorized representation of the samples of
%$\sqrt{I_{\mathcal{L}}}$ at pixel locations. $\Fbf \in \C^{N
%\times N}$ is the discrete Fourier transform (DFT) matrix, $\Pbf \in \R^{N
%\times N}$ is a binary diagonal matrix that representing the response of the
%microscope, $\Slbf \in \R^{N \times N}$ is a shift matrix specified by
%$\xibf_{\ell}$, and $\widehat{\sbf} \in \C^N$ is the vectorized discrete
%Fourier transform of the transmission function. 

%-------------------------------------------------------------------------------
\subsection{Proposed Reconstruction Algorithm}
%-------------------------------------------------------------------------------
We now propse a new reconstruction algorithm to recover the sample's amplitude
and phase maps. Let us denote the total number of measurements by $N_{\rm
img}$. We define the following optimization problem: 
\begin{equation}
  \widehat{\sbf}^{\star} = \arg \underset{\widehat{\sbf}}{\min}
  \sum_{i=1}^{N_{\rm img}} \Bigg \| \ybf_{\mathcal{L}_i} - \sqrt{\sum_{\ell \in
  {\mathcal{L}_i} } \,\bigl \lvert \Fbf \cT \Pbf \Slbf \sbf \bigr \lvert^2}
  \Bigg \|_2^2 
  \label{eq:costFunction}
\end{equation}

\section{Reconstruction Algorithm: Accelerated Wirtinger Flow}
In this section we discuss our reconstruction algorithm for recovering the sample's amplitude and phase maps from the multiplex illumination measurements. To this aim, it is natural to use the following optimization problem
\begin{align}
\label{opt}
&\underset{\vct{s}\in\C^{N_1\times N_2}}{\text{minimize}}\quad \mathcal{C}(\vct{s})\quad\text{with}\nonumber\\
&\quad\quad\mathcal{C}(\vct{s}):=\sum_{k=1}^K \fronorm{\ybf_{\mathcal{L}_k} - \sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2} }^2
%\sum_{i=1}^{n_1}\sum_{j=1}^{n_2}\ell\left(\sqrt{\mtx{I}^{(k)}_{i,j}},\abs{[\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)]_{ij}}\right).%\mathcal{R}(\vct{z})\le \mathcal{R}(\vct{x}).
\end{align}
Here, $K$ represents the total number of captured multiplexed images. We note that the above cost measures the discrepancy between the measurements and the output of the model given by \eqref{eq:discreteForwardModel}. A natural approach to solve this problem is via gradient descent type updates of the form
%\begin{align*}
%\mathcal{K}=\{\vct{w}\in\R^n:\mathcal{R}(\vct{w})\le \mathcal{R}(\vct{x})\}.
%\end{align*}
\begin{align}
\label{iters}
\vct{s}_{\tau+1}=\vct{s}_\tau-\mu_\tau\nabla \mathcal{C}(\vct{s}_\tau),
\end{align}
with $\mu_\tau$ the learning rate. We note that since $\mathcal{C}(\vct{s})$ is a mapping from $\mathbb{C}^{n_1\times n_2}$ to $\R$, it is not holomorphic and hence not complex-differentiable. However, it is still possible to define a gradient based on the notion of Wirtinger derivatives.  Following \cite{WF} we shall refer to the iterates \eqref{iters} as Wirtinger Flow. The loss function in \eqref{opt} is not differentiable and a-priori it may not be clear how to run Wirtinger Flow in this case. However, this does not pose a fundamental challenge as the loss function is differentiable except for isolated points and we can use the notion of generalized gradients to define the gradient at a non-differentiable point as one of the limits points of the gradient in a local neighborhood of the non-differentiable point. For the loss in \eqref{opt} the generalized gradient takes the form
\begin{align}
\label{gengrad}
&\nabla \mathcal{L}(\vct{s}):=\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\widetilde{\mathcal{S}}_{\ell}\left(\bar{\vct{p}}\odot \Fo_{n_1\times n_2}\left(\vct{e}\right)\right)\quad\text{where}\nonumber\\
&\vct{e}=\left(\sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2}-\ybf_{\mathcal{L}_k} \right)\odot\nonumber\\
&\quad\quad\left(\frac{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}{\sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2}}\right).
%&\sum_{k=1}^K \bar{\vct{p}}_k\odot\mathcal{F}^*\left(\left(\sqrt{\mtx{I}^{(k)}}-\abs{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}\right)\odot\frac{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}{\abs{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}}\right).
\end{align}
%%\begin{algorithm}[t]
%%    \caption{Accelerated Wirtinger Flow (AWF)}
%%    \label{AWF}
%%    \begin{algorithmic}
%%    \STATE{\bfseries Input:} Measurements $\ybf_{\mathcal{L}}$, Fourier transform of the probe $\vct{p}$ and center shifts $\xibf_\ell$ for different displacements of the probe. 
%%    \STATE {\bfseries Parameters:} $T$ iterations ($\tau$)
%%   \STATE {\bfseries Initialize:}  $\vct{s}_1=\vct{1}_{N_1\times N_2}$ or a random matrix
%%   \FOR{$\tau=1$ \textbf{to} $T$}
%%   \STATE 
%%   \vspace{-0.5cm}
%%   \begin{align*}
%%   \vct{s}_{\tau+1}\leftarrow&\vct{s}_\tau+\beta_\tau\left(\vct{s}_\tau-\vct{s}_{\tau-1}\right)\\
%%   &\quad\quad\quad-\mu_\tau\nabla \mathcal{C}\left(\vct{s}_\tau+\beta_\tau\left(\vct{s}_\tau-\vct{s}_{\tau-1}\right)\right)
%%   \end{align*}
%%   \STATE with 
%%   \vspace{-0.5cm}
%%\begin{align*}
%%&\nabla \mathcal{L}(\vct{s}):=\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\widetilde{\mathcal{S}}_{\ell}\left(\bar{\vct{p}}\odot \Fo_{n_1\times n_2}\left(\vct{e}\right)\right)\quad\text{where}\nonumber\\
%%&\vct{e}=\left(\sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2}-\ybf_{\mathcal{L}_k} \right)\odot\nonumber\\
%%&\quad\quad\left(\frac{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}{\sqrt{\sum_{\ell \in \mathcal{L}_k} \,\abs{\Fo_{n_1\times n_2}^{-1}\left(\mtx{p}\odot \mathcal{S}_\ell(\mtx{s})\right)}^2}}\right),
%%%&\sum_{k=1}^K \bar{\vct{p}}_k\odot\mathcal{F}^*\left(\left(\sqrt{\mtx{I}^{(k)}}-\abs{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}\right)\odot\frac{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}{\abs{\mathcal{F}\left(\vct{p}_k\odot \vct{z}\right)}}\right).
%%\end{align*}
%%   \STATE 
%%   $\beta_\tau=\frac{\tau+1}{\tau+3},$ and
%%   $\mu_\tau = \frac{1}{ \infnorm{\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}\odot \abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}}}$.
%%   \ENDFOR 
%%    \STATE{\bfseries Output:} $\vct{s}_T$
%%    \end{algorithmic}
%%  \end{algorithm}
Here, $\bar{\mtx{p}}\in\C^{n_1\times n_2}$ is a matrix whose entries are the conjugate of the entries of $\mtx{p}$ and $\Fo_{n_1\times n_2}:\C^{n_1\times n_2}\rightarrow \C^{n_1\times n_2}$ represents the $n_1\times n_2$ two dimensional discrete Fourier transform. Also, $\widetilde{\mathcal{S}}_\ell:\C^{n_1\times n_2}\rightarrow \C^{N_1\times N_2}$ is a mapping that when applied to $\mtx{x}\in\C^{n_1\times n_2}$ creates an all zero matrix of size $N_1\times N_2$ except for a submatrix of size $n_1\times n_2$ with center located at position $\xibf_{\ell}$ which is set to $\vct{x}$. Furthermore, for two matrices $\mtx{A}$ and $\mtx{B}$ of the same size $\frac{\mtx{A}}{\mtx{B}}$ is used to denote element-wise division. In particular, $\frac{\mtx{A}}{\abs{\mtx{A}}}$ is a matrix whose entries contain the phase of the entries of the matrix $\mtx{A}$. We propose the following step size for the Wirtinger Flow iterates
\begin{align}
\label{step1}
\mu_\tau =\mu:=\frac{1}{ \infnorm{\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}\odot \abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}}}.
\end{align}
Here, for a matrix $\mtx{A}$, $\infnorm{\mtx{A}}$ denotes the maximum absolute value of the entries of $\mtx{A}$ i.e.~$\infnorm{\mtx{A}}:=\max_{ij}\abs{\mtx{A}_{ij}}$. We shall demonstrate in Section \ref{Sec:NumericalResults} that the Wirtinger Flow iterates \eqref{iters} using the generalized gradient in \eqref{gengrad} enjoys faster convergence when compared with many classical phase retrieval schemes. This result holds with the step size \eqref{step1}. However, the convergence rate is still rather slow. To overcome this challenge, inspired by \cite{} we apply the accelarted iterations
\begin{align}
\label{AWF}
\vct{s}_{\tau+1}=\vct{s}_\tau+\beta_\tau\left(\vct{s}_\tau-\vct{s}_{\tau-1}\right)-\mu_\tau\nabla \mathcal{C}\left(\vct{s}_\tau+\beta_\tau\left(\vct{s}_\tau-\vct{s}_{\tau-1}\right)\right).
\end{align}
Following \cite{} we shall refer to these iterations as Accelarated Wirtinger Flow (AWF). We also propose the following values for the parameters $\beta_\tau$ and $\mu_\tau$ so that our approach requires no tuning parameters
\begin{align}
\label{params}
\beta_\tau=&\frac{\tau+1}{\tau+3}\quad\text{and}\quad\nonumber\\
\mu_\tau =&\mu:=\frac{1}{ \infnorm{\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}\odot \abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}}}.
\end{align}
%We summarize this approach in Algorithm \ref{AWF}.

We note that Nesterov's accelerated scheme applies to convex and smooth functions. However, the loss function in \eqref{opt} is neither convex nor differentiable. Therefore, a-priori it is not clear why such an accelerated scheme is useful. Perhaps unexpectedly, we shall demonstrate in Section \ref{Sec:NumericalResults} that these accelerated iterates not only enjoy much faster convergence but also reach better optima!

\section{Theory for convergence to stationary points}
\label{sectheory}
In this section we wish to provide some theoretical justification for our choice of the learning rates \eqref{step1} and \eqref{params} for Wirtinger Flow and Accelerated Wirtinger Flow.
\begin{theorem}\label{mainthm} For $k=1,2,\ldots,K$, let $\ybf_{\mathcal{L}_k}\in\mathbb{R}^{n_1\times n_2}$ denote arbitrary measurements. Also let $\vct{p}\in\mathbb{C}^{n_1\times n_2}$ denote the discretized Fourier transform of the probe. We run the Wirtinger Flow updates
\begin{align*}
\vct{s}_{\tau+1}=\vct{s}_\tau-\mu_\tau\nabla\mathcal{C}(\vct{s}_\tau),
\end{align*}
with $\nabla \mathcal{C}(\vct{s})$ as defined in \eqref{gengrad} and learning rate $\mu_\tau$  obeying
\begin{align}
\label{stepthm}
\mu_\tau =\mu:=\frac{1}{ \infnorm{\sum_{k=1}^K\sum_{\ell\in\mathcal{L}_k}\abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}\odot \abs{\widetilde{\mathcal{S}}_{\ell}(\vct{p})}}}.
\end{align}
Also let $\vct{s}_{*}\in\underset{\vct{s}\in\C^{N_1\times N_2}}{\arg\min} \mathcal{C}(\vct{s})$ be a global optima. Then, the following identities hold
\begin{align*}
\underset{\tau\rightarrow\infty}{\lim} \fronorm{\nabla \mathcal{C}(\vct{s}_\tau)}\rightarrow 0,
\end{align*}
and
\begin{align*}
\min_{\tau\in\{1,2,\ldots,T\}} \fronorm{\nabla \mathcal{C}(\vct{s}_\tau)}^2\le \frac{\left(\mathcal{C}(\vct{s}_1)-\mathcal{C}(\vct{s}_{*})\right)}{\mu T}.
\end{align*}
\end{theorem}
This theorem demonstrates that with our chosen step size the Wirtinger Flow iterates converge to a point where the generalized gradient is zero. This is a non-trivial statement as the loss function is none smooth and there are many stationary points where the generalized gradient does not vanish. The main use of this theorem in this paper is that it allows us to select the learning rate properly. We would like to note that this theorem does not show convergence to a local optimum. Furthermore, this theorem does not provide convergence guarantees for Accelerated Wirtinger Flow. We hope to address such questions in our future work. 

